Monocular and Stereo Cues for Landing Zone Evaluation for Micro UAVs

Autonomous and safe landing is important for unmanned aerial vehicles. We present a monocular and stereo image based method for fast and accurate landing zone evaluation for UAVs in various scenarios. Many existing methods rely on Lidar or depth sensor to provide accurate and dense surface reconstruction. We utilize stereo images to evaluate the slope and monocular images to compute homography error. By combining them together, our approach works for both rigid and non-rigid dynamic surfaces. Experiments on many outdoor scenes such as water, grass and roofs, demonstrate the robustness and effectiveness of our approach.

==> inputs/0_asbtract.tex <==
Safe landing of autonomous UAVs requires a reliable perception system. The proposed approach provides robust feedback about the landing surface through monocular and stereo based methods. A dense terrain reconstruction using stereo and inertial data assesses slope and roughness, and a fast, monocular approach detects the presence of non-rigid surfaces such as water or grass. The performance of this approach is demonstrated on a micro-UAV over a variety of terrains.





keywords: UAV, stereo, monocular, landing

==> inputs/draft_space.tex <==
\begin{table}[ht]
\centering
 \begin{tabular}{||c | c | c | c | c | c |} 
 \hline
 Scene & BM & BM + WLS + LRC & SGBM & SGBM + WLS + LRC & LIBELAS \\ [0.5ex] 
 \hline\hline
 Scene 1 & 33.3\% & 30.3\% & 18\% & 16.2\% & 9.8\%  \\ 
 \hline
 Scene 2 & 37.6\% & 36.5\% & 21.8\% & 20.9\% & 20.2\%  \\
 \hline
 Scene 3 & 37.4\% & 36.2\% & 18.8\% & 17.6\% & 12.6\%  \\
 \hline
 Scene 4 & 39.1\% & 39.5\% & 17.6\% & 16.6\% & 9.1\%  \\
 \hline
 Scene 5 & 42.5\% & 37.2\% & 17.8\% & 16.0\% & 23.7\%  \\
 \hline
 Scene 6 & 67.0\% & 53.2\% & 33.1\% & 31.5\% & 40.4\%  \\
 \hline
 Scene 7 & 70.0\% & 58.3\% & 30.2\% & 28.8\% & 40.5\%  \\
 \hline
 Scene 8 & 49.2\% & 45.5\% & 35.3\% & 34.4\% & 32.4\%  \\
 \hline
 Scene 9 & 54.0\% & 50.5\% & 35.8\% & 35.3\% & 29.4\%  \\
 \hline
 Scene 10 & 57.3\% & 48.7\% & 38.7\% & 36.0\% & 31.7\%  \\ [1ex] 
 \hline
\end{tabular}
\caption{Percentage bad pixels (error $> 4$)}
\label{tab:bad_4}
\end{table}

\begin{table}[ht]
\centering
 \begin{tabular}{||c | c | c | c | c | c |} 
 \hline
 Scene & BM & BM + WLS + LRC & SGBM & SGBM + WLS + LRC & LIBELAS \\ [0.5ex] 
 \hline\hline
 Scene 1 & 49.7\% & 46.5\% & 36.7\% & 35.3\% & 32.2\%  \\ 
 \hline
 Scene 2 & 52.0\% & 51.2\% & 39.8\% & 39.3\% & 40.6\%  \\
 \hline
 Scene 3 & 49.5\% & 48.3\% & 32.8\% & 31.7\% & 36.3\%  \\
 \hline
 Scene 4 & 53.0\% & 54.2\% & 34.6\% & 33.1\% & 28.6\%  \\
 \hline
 Scene 5 & 56.4\% & 52.5\% & 35.8\% & 34.9\% & 44.4\%  \\
 \hline
 Scene 6 & 75.1\% & 66.4\% & 57.3\% & 55.6\% & 57.5\%  \\
 \hline
 Scene 7 & 79.6\% & 71.0\% & 56.1\% & 57.3\% & 60.1\%  \\
 \hline
 Scene 8 & 62.8\% & 63.6\% & 53.9\% & 53.8\% & 50.0\%  \\
 \hline
 Scene 9 & 68.1\% & 67.0\% & 56.5\% & 56.3\% & 47.9\%  \\
 \hline
 Scene 10 & 69.8\% & 65.9\% & 58.7\% & 58.3\% & 50.0\%  \\ [1ex] 
 \hline
\end{tabular}
\caption{Percentage bad pixels (error $> 2$)}
\label{tab:bad_2}
\end{table}

Autonomous landing for drones is becoming increasingly important with their rising use across different environments and operating conditions. The system developed in this paper aims to provide a robust, real-time landing zone evaluation algorithm that provides information on the landing site in terms of terrain slope, roughness as well as being able to identify non-rigid surfaces such as water and grass. Initial experiments show the computational feasibility of the proposed approach as well as demonstrate the robustness to varying scenes.

References for full paper literature review section:
1. Vision Guided Landing of an Autonomous Helicopter in Hazardous Terrain
Andrew Johnson, James Montgomery and Larry Matthies
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=1570727

2. Autonomous Detection of Safe Landing Areas for an UAV from Monocular Images
Sebastien Bosch ;  Simon Lacroix ;  Fernando Caballero
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=4059308

3. The Jet Propulsion Laboratory Autonomous Helicopter Testbed: A Platform for Planetary Exploration Technology Research and Development
James F. Montgomery and Andrew E. Johnson, Stergios I. Roumeliotis, Larry H. Matthies
https://onlinelibrary.wiley.com/doi/epdf/10.1002/rob.20110

4. Autonomous Vision-based Landing and Terrain Mapping Using an MPC-controlled Unmanned Rotorcraft
Todd Templeton, David Hyunchul Shim, Christopher Geyer, and S. Shankar Sastry
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=4209276

5. Vision Based Terrain Recovery for Landing Unmanned Aerial Vehicles
Marci Meingast, Christopher Geyer, and Shankar Sastry
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=1430284

6. Flight Trials of a Rotorcraft Unmanned Aerial Vehicle Landing Autonomously at Unprepared Sites
Colin Theodore, Adnan Ansar
https://www.researchgate.net/profile/Adnan_Ansar/publication/252103988_Flight_Trials_of_a_Rotorcraft_Unmanned_Aerial_Vehicle_Landing_Autonomously_at_Unprepared_Sites/links/546f840e0cf24af340c08f91/Flight-Trials-of-a-Rotorcraft-Unmanned-Aerial-Vehicle-Landing-Autonomously-at-Unprepared-Sites.pdf


==> template/referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O�Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...�': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

